Prediction-Constrained Training for Semi-Supervised Mixture and Topic Models

Supervisory signals have the potential to make low-dimensional data representations, like those learned by mixture and topic models, more interpretable and useful. We propose a framework for training latent variable models that explicitly balances two goals: recovery of faithful generative explanations of high-dimensional data, and accurate prediction of associated semantic labels. Existing approaches fail to achieve these goals due to an incomplete treatment of a fundamental asymmetry: the intended application is always predicting labels from data, not data from labels. Our prediction-constrained objective for training generative models coherently integrates loss-based supervisory signals while enabling effective semi-supervised learning from partially labeled data. We derive learning algorithms for semi-supervised mixture and topic models using stochastic gradient descent with automatic differentiation. We demonstrate improved prediction quality compared to several previous supervised topic models, achieving predictions competitive with high-dimensional logistic regression on text sentiment analysis and electronic health records tasks while simultaneously learning interpretable topics.

==> Makefile <==
SHELL = /bin/bash

TMP_RESULT=$$(bash -c "find tex_for_arxiv_paper/ -name '*.tex' | xargs grep "figures/" | cut -d':' -f2 | grep -v '%'");
PDF_FIGFILE_LIST=$$(python -c "print ' '.join([s + '.pdf' * (1 - s.endswith('.pdf')) for s in [x.partition('}')[0] for x in '''$(TMP_RESULT)'''.split('{')] if s.startswith('figures/')])");

clean::
	rm -fv *.zip *.aux *.log *.bbl *.blg *.toc *.out *.lot *.lof *.dvi *.ps *.pdf

pdf_figures:
	@bash convert_eps_to_pdf.sh

### main_arxiv

src_for_arxiv.zip: main_arxiv.bbl
	zip -r src_for_arxiv.zip \
		Makefile \
		*.bbl \
		*.bib \
		arxiv_nips_2017.sty \
		main_arxiv.tex \
		tex_for_arxiv_paper/*.tex \
		$(PDF_FIGFILE_LIST)

main_arxiv: main_arxiv.pdf

main_arxiv.pdf: main_arxiv.tex main_arxiv.bbl
	# Run 3x to get cross refs right
	latex -interaction nonstopmode main_arxiv
	latex -interaction nonstopmode main_arxiv
	latex -interaction nonstopmode main_arxiv
	dvipdf main_arxiv.dvi

main_arxiv.bbl: references.bib main_arxiv.tex tex_for_arxiv_paper/*.tex
	latex -interaction nonstopmode main_arxiv
	bibtex main_arxiv

### main_nips

main_nips: main_nips.pdf

main_nips.pdf: main_nips.tex main_nips.bbl
	# Run 3x to get cross refs right
	latex -interaction nonstopmode main_nips
	latex -interaction nonstopmode main_nips
	latex -interaction nonstopmode main_nips
	dvipdf main_nips.dvi

main_nips.bbl: references.bib main_nips.tex tex_for_nips_paper/*.tex
	latex -interaction nonstopmode main_nips
	bibtex main_nips

### main_nips_supplement

main_nips_supplement: main_nips_supplement.pdf

main_nips_supplement.pdf: main_nips_supplement.tex main_nips_supplement.bbl
	# Run 3x to get cross refs right
	latex -interaction nonstopmode main_nips_supplement
	latex -interaction nonstopmode main_nips_supplement
	latex -interaction nonstopmode main_nips_supplement
	dvipdf main_nips_supplement.dvi

main_nips_supplement.bbl: references.bib main_nips_supplement.tex tex_for_nips_supplement/*.tex
	latex -interaction nonstopmode main_nips_supplement
	bibtex main_nips_supplement

